Adversarial Resilience in Sequential Prediction via Abstention

We study the problem of sequential prediction in the stochastic setting with an adversary that is allowed to inject clean-label adversarial (or out-of-distribution) examples. Algorithms designed to handle purely stochastic data tend to fail in the presence of such adversarial examples, often leading to erroneous predictions. This is undesirable in many high-stakes applications such as medical recommendations, where abstaining from predictions on adversarial examples is preferable to misclassification. On the other hand, assuming fully adversarial data leads to very pessimistic bounds that are often vacuous in practice. To capture this motivation, we propose a new model of sequential prediction that sits between the purely stochastic and fully adversarial settings by allowing the learner to abstain from making a prediction at no cost on adversarial examples. Assuming access to the marginal distribution on the non-adversarial examples, we design a learner whose error scales with the VC dimension (mirroring the stochastic setting) of the hypothesis class, as opposed to the Littlestone dimension which characterizes the fully adversarial setting. Furthermore, we design a learner for VC dimension~1 classes, which works even in the absence of access to the marginal distribution. Our key technical contribution is a novel measure for quantifying uncertainty for learning VC classes, which may be of independent interest.

==> A-proofs.tex <==

\section{Proofs from \cref{sec:known_marg}}
\label{app:proofs4}

\subsection{Properties of Higher-Order Disagreement: Proof of \cref{lem:prob_abs}}

We first begin by relating the probabilities of shattering $k$ points for the classes gotten by restricting to evaluating to $0$ and $1$ at $x$ respectively, for an arbitrary point $x$.
The proof of the following lemma uses a simple inclusion exclusion argument.
    
\begin{lemma} \label{lem:beta}
    For all $x \in \dom $ and any hypothesis class $\cls$, we have
    \begin{align}
        \dist^{\otimes k} \left( \dis \left( \clswpointo \right) \right) + \dist^{\otimes k} \left( \dis \left( \clswpointz \right) \right) \leq \dist^{\otimes k} \left( \dis \left( \cls \right) \right) + \dist^{\otimes k} \left( \dis \left( \clswpointo   \right) \cap  \dis \left( \clswpointz \right)  \right). 
    \end{align}
Equivalently, 
\begin{equation}
    \distprob \left( \clswpointo \right) + \distprob \left( \clswpointz \right) \leq \distprob \left( \cls \right) + \Pr_{x_1, \dots , x_k \sim \dist } \left[  x_1 , \dots , x_{k} \text{ is shattered by both } \clswpointo \text{ and } \clswpointz     \right]. 
\end{equation}
\end{lemma}
\begin{proof}
    For $x_1, \dots, x_n \in \dom$, consider the four indicator random variables given by 
    \begin{align}
        A_1 &= \mathbbm{1}  \left(  x_1, \dots , x_n \text{ is shattered by } \clswpointo \right) \\ 
        A_2 &= \mathbbm{1} \left(  x_1, \dots , x_n \text{ is shattered by } \clswpointz \right) \\ 
        A_3 &= \mathbbm{1} \left(  x_1, \dots , x_n \text{ is shattered by } \clswpointo \text{ and } \clswpointz \right) \\
        A_4 &= \mathbbm{1} \left(  x_1, \dots , x_n \text{ is shattered by } \cls \right). 
    \end{align}
    Note that $  A_1 + A_2 \leq A_3 + A_4 $. 
    Taking expectations gives the desired result.
\end{proof}

In order to prove the main lemma, we then take expectations with respect to the point $x$ drawn independently from $\dist$.
The key observation is to relate the probability of $k$ point being shattered by both classes that evaluate to $0$ and $1$ at $x$, for a random point $x$, to the probability of shattering $k+1$ points.

\begin{proof}[Proof of \cref{lem:prob_abs}]
    The proof follows by using \cref{lem:beta} to get \cref{eq:lemapp} and Markov's inequality to get \cref{eq:markov}. 
    The final line follows by noting that since $x_1, \dots , x_k$ and $x$ are drawn from $\dist$ and are shattered, \cref{eq:markov} computes the probability that $k+1$ points are shattered. 
    \begin{align}
        &\Pr_{x \sim \dist } \left[ \distprob\left( \clswpointz \right) + \distprob\left( \clswpointo \right) \geq  2\eta  \distprob\left( \cls \right)  \right] \\
        \leq &\Pr_{x \sim \dist }\left[ \distprob \left( \cls \right) + \Pr_{x_1, \dots , x_k \sim \dist } \left[  x_1 , \dots , x_{k} \text{ is shattered by both } \clswpointo \text{ and } \clswpointz     \right]  \geq   2\eta  \distprob \left( \cls \right)   \right]  \label{eq:lemapp} \\ 
        \leq &\Pr_{x \sim \dist} \left[  \Pr_{x_1, \dots , x_k \sim \dist } \left[  x_1 , \dots , x_{k} \text{ is shattered by both } \clswpointo \text{ and } \clswpointz     \right]  \geq  \left(  2\eta - 1 \right)  \distprob \left( \cls \right)   \right] \\ 
        \leq &\frac{ \cdot \mathbb{E} \left[ \Pr_{x_1, \dots , x_k \sim \dist } \left[  x_1 , \dots , x_{k} \text{ is shattered by both } \clswpointo \text{ and } \clswpointz     \right] \right] }{    \left( 2\eta - 1 \right)\distprob \left( \cls  \right) } \label{eq:markov} \\ 
        \leq &\frac{1}{ 2\eta - 1 }  \cdot \frac{ \distprob[k+1] \left( \cls  \right)  }{  \distprob{} \left( \cls  \right) }. 
    \end{align}
\end{proof}




\subsection{Proof of \cref{lem:non_abs_err}} \label{sec:non_abs_err}

\begin{proof}
Note that from definition of Algorithm \ref{alg:abstention}, we have that when $ \pred \neq \bot $,  $ \min \left\{ \distprob{} \left( \clstwpointo \right) , \distprob{} \left( \clstwpointz \right)  \right\}  \leq 0.6  \distprob{} \left( \clst  \right) $.
Thus, since we predict with the label corresponding to $\max \left\{ \distprob{} \left( \clstwpointo \right) , \distprob{} \left( \clstwpointz \right)  \right\} $, if we make a mistake, we have 
\begin{align}
    \distprob{} \left( \clst[t+1] \right) \leq 0.6 \cdot \distprob{} \left( \clst[t] \right). 
\end{align}


Also, note once end of the phase corresponding to $k$, $ \kintend $, is reached when $ \distprob{} \left( \clst \right) \leq \alpha_k $. 
This leads to the required bound. 
\end{proof}


\subsection{Proof of \cref{lem:abs_err}} \label{sec:abs_err}


\begin{proof}
    Let $t\in [\ell_k, m_k]$.
    Recall that $\clst$ denotes the class consistent with the data seen till time $t$.
    Recall that $H_t$ denotes the history of the interaction till time $t$.

    

\begin{align}
     \mathbb{E} \left[   \mathbbm{1} \left[ \corrind = 0 \land \pred \left( \postcorsamp \right)  = \bot \right]  \mid \hist  \right] & = \mathbb{E} \left[   \mathbbm{1} \left[ \corrind = 0 \land \pred \left( \precorsamp \right)  = \bot \right]  \mid \hist  \right]  \label{eq:repcorr}  \\
     & \leq \mathbb{E} \left[   \mathbbm{1} \left[ \pred \left( \precorsamp \right)  = \bot \right]  \mid \hist  \right] \label{eq:dropcond}   \\ 
     & \leq \Pr \left[ \min\left\{ \distprob \left( \clstwpointo  \right) , \distprob \left( \clstwpointo  \right) \right\} \geq 0.6 \distprob \left( \clst \right)  \mid \hist \right] \label{eq:repwithprob}    \\
     & \leq \Pr \left[  \distprob \left( \clstwpointo  \right) + \distprob \left( \clstwpointo  \right) \geq 1.2 \distprob \left( \clst \right)  \mid \hist \right] \label{eq:minsum}   \\
     & \leq 5 \frac{ \distprob[k+1] \left( \clst \right)  }{\distprob[k] \left( \clst \right)} \label{eq:usinglem}    \\ 
     & \leq 5 \frac{\alpha_{k+1}}{ \alpha_k}  \label{eq:finalstep}  . 
\end{align}
The equality in \cref{eq:repcorr} follows from the fact that in the uncorrupted rounds, $ \postcorsamp = \precorsamp $.
The inequality in \cref{eq:repwithprob} follows from the condition for abstention in Algorithm \ref{alg:abstention} and the fact that $\precorsamp \sim \dist $.
\cref{eq:minsum} follows from the fact that the min of two numbers is at most their average. 
The key step is \cref{eq:usinglem} which follows from \cref{lem:prob_abs}.
\cref{eq:finalstep} follows from the fact that at level $k$ in Algorithm \ref{alg:abstention}, $ \distprob[k+1] \left( \clst \right) \leq \alpha_k $ and $ \distprob \left( \clst \right) \geq \alpha_{k+1} $.    


Summing this bound and noting that $ \kintend - \kintstart $ is at most $ T $, we get the required bound.








\end{proof}


\subsection{Proof of \cref{thm:abstention}}

\begin{proof}
    
    
    
    First, let us look at the misclassication error. 
    Note that Algorithm \ref{alg:abstention} will not misclassify when $k=1$.
    To see this, recall from \cref{def:dis} that  $ \postcorsamp \not  \dis[1] $ implies that there is a unique label consistent with the history. 
    For the remaining levels, we sum the errors from \cref{lem:non_abs_err} and recall that $ \alpha_k = T^{-k} $, which gives us 
    \begin{align}
        \mathsf{Misclassification Error} &=  {\sum_{t =1}^T \mathbbm{1}[\hat{y}_t = 1 - f^\star(x_t)]} \\ 
        &\leq 2 \sum_{k=2}^d \log\left( \frac{1}{ \alpha_k } \right) \\ 
        & \leq 2 \sum_{k=2}^d k \log T \\ 
        &\leq d^2 \log T.
    \end{align}
    

    
    
    For the abstention error, we again begin with the case of $k=1$.
    Note that for $t \geq \kintstart[1] $, we have 
    
    \begin{align}
        \Pr_{x \sim \dist } \left[ x \in \dis[1] \left( \clst \right)   \right] \leq \kthres[1]. 
    \end{align}
    Thus, we have a bound of $ T \kthres[1] \leq 1  $ on the expected error in this case.
    For the remaining levels, we sum the error from \cref{eq:abs_err} over all $k$, which gives us the bound
    \begin{align}  
        \mathsf{Abstention Error} &= {\sum_{t =1}^T\mathbbm{1}[c_t = 0 \land \hat{y}_t = \perp]} \\ 
        & = \sum_{k=1}^d \mathbb{E} \left[ \sum_{t = \kintstart }^{\kintend}  \mathbbm{1} \left[ \corrind  = 0 \land \pred  = \bot  \right] \right] \\ 
        &= 1 + 5T \sum_{k=2}^d \frac{ \alpha_{k+1} }{ \alpha_k } \\ 
        & = 1 + 5T \sum_{k=2}^d \frac{ 1 }{ T }   \\ 
        & \leq 5d + 1 \\ 
        & \leq 6d.
    \end{align}
    This gives us the desired bounds.
    
    
    











\end{proof}

==> B-proofs.tex <==
\section{Proofs from \cref{sec:unknown_dist}}
\label{app:proofs5}
\subsection{Structure for VC Dimension One Classes}

    \begin{definition}
        Consider a domain $\dom$ and a partial order $\prec$ on $\dom$.
        We say that a set $I$ is an initial segment of $\prec$ if for all $x \in I$ and $y \in \dom$ such that $y \prec x$, we have $y \in I$.  
        We say that a partial order is a tree ordering if every initial segment $I$ is a linear order i.e. for all $x,y \in I$, either $x \prec y$ or $y \prec x$.
    \end{definition}


    \begin{theorem}[\cite{bendavid20152}] \label{lem:vc_char} 
        Let $\cls$ be a hypothesis class over the domain $\dom$.
        Then, the following are equivalent:
        \begin{enumerate}
            \item[a.] $\cls$ has VC dimension $1$.
            \item[b.] There is a tree ordering $\prec$ on $\dom$ and a hypothesis $f \in \cls$ such that every element of the set 
            \begin{align}
                \cls_f = \left\{ h \oplus f : h \in \cls    \right\}
            \end{align} 
            is an initial segment of $\prec$.
        \end{enumerate}
    \end{theorem}

    The result above was initially observed in \cite{bendavid20152}. 


    
    

    \subsection{Proof of \cref{lem:unknown_misclass_bound} } \label{sec:unknown_misclass_bound} 

    \begin{lemma} \label{lem:mistboundgamma}
    For any $t$, we have that
    
    \begin{align} \label{eq:mistboundgamma}
        \loonum_{t+1} \leq \loonum_t - \alpha \cdot \mathbbm{1} \left[ \text{Misclassification at time } t  \right] + 1 . 
    \end{align}
\end{lemma}

    
    \begin{proof}
        First, note that in any round that a mistake was not made, we have that $ \loonum_{t+1} \leq \loonum_t + 1 $. 
        This is because at most one point is added to the data set in each round.
 
        Note that $ \abs{ \looset \left( \data[t-1] , \clswpointz[\postcorsamp{}][1]   \right)   }  +  \abs{ \looset \left( \data[t-1] , \clswpointo[\postcorsamp{}][0]   \right)   } \leq \abs{ \looset \left( \data[t-1] , \cls   \right)   }    $. 
        Further, we have $ \abs{ \looset \left( \data , \cls \right) } \leq    \abs{ \looset \left( \data[t-1] , \clswpointz[\postcorsamp{}][y_t]   \right)   } +1  $. 
        From the condition for predicting, we have that $  \max\left\{  \abs{ \looset \left( \data[t-1] , \clswpointz[\postcorsamp{}][1]   \right)   }  ,  \abs{ \looset \left( \data[t-1] , \clswpointo[\postcorsamp{}][0]   \right)   }  \right\}  \geq \alpha  $. 
     
     Since if we make a misclassication, we go to the smaller value for $ \looset$, we get the desired bound.   
     \end{proof}



     \begin{proof}
        Note that $ \mathsf{Misclassification Error} = \sum_{t=1}^T \mathbbm{1} \left[ \text{Misclassification at time } t  \right] $. 
        Rearranging \eqref{eq:mistboundgamma} and summing gives us 
        \begin{align}
            \mathsf{Misclassification Error} \leq \frac{1}{ \alpha} \sum_{t=1}^{T} \left( \loonum_t - \loonum_{t+1} +1 \right)           
        \end{align}
        Note that for all $i$, we have that $ \loonum_i \leq T$ which gives us the desired bound. 
    
    
    
    
    \end{proof}

    \subsection{Proof of \cref{lem:abstention_unknown} }
     

    \begin{definition}[Attackable Point]
    \label{def:atackable}
    Let $\cls$ be a hypothesis class and let $f \in \cls $ be a representative function.
    Let $S$ be a realizable dataset. 
    We say that a point $x$ is attackable with respect to a data set $S$ if there exists is a sequence of adversarial examples $ A_x $ such that algorithm abstains on example  $ x    $ when the history is $ S \cup A_x \backslash \left\{ x \right\}  $. 
    In other words, $x$ is attackable if there is a set of adversarial examples $A_x$ such that $x \notin  \dis[1] \left(  \clsrestS[ \cls ][S \cup A_x \backslash \left\{ x \right\}]  \right) $ and
    \begin{align}
        \max \left\{ \abs{ \looset \left( S \cup  A_x \backslash \left\{ x \right\} , \clswpointz[x{}][ 0  ]   \right)   } ,   \abs{ \looset \left( S \cup A_x \backslash \left\{ x \right\} , \clswpointz[x{}][ 1  ]   \right)   }    \right\}  \leq \alpha . 
    \end{align} 
\end{definition}


    The key lemma for our analysis is that the number of attackable examples is bounded. 


    \begin{lemma}  \label{lem:attackable}
        Let $\cls$ be a hypothesis and $f \in \cls $ be any reference function.
        Let $ S $ be any set of examples.
        Then, the number of attackable examples is at most $ \alpha $. 
    \end{lemma}
    
    The proof uses a structure theorem for classes with VC dimension one which states that they can be represented as initial segements of a tree order. 



    
     \begin{proof}
             Let $f$ be the representative function from the characterization in \cref{lem:vc_char}. 
        Futher, let $ \mathfrak{T} $ be the tree corresponding to the tree order on $ \mathcal{X} $. 
        Since $f$ is a fixed function that does not depend on the algorithm or the history of interaction with adversary, we can preprocess all points and labels to be xored with the labels of $ f $. 
        In other words, we tranform the class to be such that $f$ is the all zeros function.
        In this setting, the true hypothesis $ f^{\star} $ corresponds to a path $p$ and a threshold $ x^{\star} $ on $ \mathfrak{T} $ such that $ f^{\star} (x) =1  $ if and only if $ x \in p $ and $ x \prec x^{\star} $.
        For this proof, it is important to consider only adversaries that do not get to chose the true hypothesis $ f^{\star} $ adaptively. 
        Thus the path is fixed throughout the history of the interaction. 

            Let $S$ be the data set under consideration. 
        First note that by definition, we only need to consider the points $x$ in the disagreement region. 
        The labels of all points that are not in the subtree of the deepest $1$ labeled point in $S$ are fixed and thus cannot be in the disagreement region.
        Thus, we only need to consider the points in the subtree of the deepest $1$ labeled point in $S$. 
        

             First note that points that have more than $ \alpha $ points in descendant subtree cannot be attacked. 
        This is because if the point is labelled as a $0$ then all its descendants are in the disagreement region. 
        This remains true even for any points that are added to the data set.
        Thus, $\abs{ \looset \left( S \cup  A_x \backslash \left\{ x \right\} , \clswpointz[x{}][ 0  ]   \right)   } > \alpha  $. 
        This is because in the definition of $\loonum$ we remove all points labelled $0$.

             For any node $u$, denote by $ \mathrm{pos }(v) $ the closest ancestor on the path $p$ corresponding to the positive points. 
        We claim that if $u$ has fewer than $ \alpha $ points in its descendant subtree, then $u$ is attackable only if
        \begin{align} \label{eq:attackable} 
            \abs{  \left\{ v \in S :  \mathrm{pos}(u) \preceq \mathrm{pos}(v)  \land v \text{ is not a descendant of } u  \right\}  } \leq \alpha 
        \end{align}
        
        
        
        First note that adding any $0$ labelled points to $S$ as $A_u$ does not change the number of points in $ \looset  $. 
        Further note that for $v$ such that $ \mathrm{pos}(u) \preceq \mathrm{pos}(v)$, adding a $1$ labelled point must be on the path between $\mathrm{pos}(u)$ and $\mathrm{pos}(v)$.
        But, this would remove $u$ from the disagreement region.
        Thus, all point $v$ would be counted in $ \looset $  and if these are greater than $\alpha $ then $u$ is not attackable. 
        
        
        

        
        
        Consider the point $w$ that is minimal amongst $  \mathrm{pos}(u) $ for $ u $ satisfying \eqref{eq:attackable} and $u$ be a node such that $\mathrm{pos}(u) = w $.  
        
        First note that all points that satisfy \eqref{eq:attackable} are in the subtree of $w$. 
        Second, note that this subtree has at most $ \alpha $ points. 
        This is because if there were more than $ \alpha $ points, $u$ would not satisfy \eqref{eq:attackable} which is a contradiction. 
        
     \end{proof}



    

    
    
    
    
    
    
        
    
    
    
    
    
        
    
    
    
    
        
    
    
    
    
    
    
    
    


    




    
    





       


        \begin{proof}[Proof of \cref{lem:abstention_unknown}]
            
            
            
            
            
            
            
            Let $i_T$ be the number of i.i.d. points in the data set at time $T$.
            Note that the only i.i.d. points that we abstain on are the attackable points. 
            But, since the i.i.d. points are exchangeable if $i$ i.i.d. points are seen so far, the probability of abstain is given by $\frac{\alpha}{i}.$
            Thus, the expected total number of abstentions is at most
            \begin{align}
                \sum_{i=1}^{i_T} \frac{\alpha}{i} \leq \alpha \log T
            \end{align} 
            as required. 
        \end{proof}


==> C-discussion.tex <==
\section{Discussion}

In this section, we further discuss the proposed algorithms and propose potential ways to extend these beyond the current settings. 

\subsection{Generalizing Higher-order Disagreement to Unknown Distribution}

    In \cref{sec:known_marg}, we saw an algorithm that for any class $\cls$ with VC dimension $d$, achieves abstention error and misclassification error bounded only as a function of $d$. 
    As mentioned earlier, an interesting open question is to extend this to the unknown distribution case. 
    In this section, we will briefly discuss a natural algorithm extending the algorithm from the known distribution case. 
    Recall that Algorithm~\ref{alg:abstention} computed the probabilities of shattering $k$ points using the knowledge of the distribution and made a prediction $\pred$ depending on the relative magnitudes of the probabilities corresponding to the two restricted classes.
    The main challenge in the unknown distribution case is that it is not immediately obvious how to compute these quantities. 

    One natural approach is to use the historical data as a proxy for the distribution. 
    
    That is, given the data set $\data$ of size $n$, compute the leave-$k$-out estimator for the probability as follows 
    \begin{align}
        \tilde{\rho}_k (S, \cls ) = \frac{1}{ \binom{  n}{k }  } \sum_{ T \subset S ; |T| =k    }  \mathbbm{1} \left[  T \text{ is shattered by } \cls|_{S \backslash T  }   \right] . 
    \end{align}
    
    There are a few things to observe about this estimator. 
    First, in the case when the data is generated i.i.d., this estimator is unbiased. 
    Further, though each of the summands is not independent, one can show concentration for estimators of this form using the theory of U-statistics.
    Additionally, recall that in Algorithm~\ref{alg:abstention} required the thresholds $\kthres$ to be set to $T^{-O(k)}$ (we use $T^{-k}$ but it is straightforward to extend this to $T^{-ck}$ for $c < 1$). 
    This appears to be high precision but note that the ``number of samples" one has for a data set of size $n$ is $n^{O(k)}$. 
    Thus, it is conceivable that such an estimator can give the necessary bounds. 
    Unfortunately, the challenge with analyzing this in our setting is that we do no know which of the examples are corrupted. 
    Thus, the adversary could inject examples to make our estimates arbitrarily inaccurate.
    Thus, as in the case of the VC dimension 1 classes we saw in \cref{sec:unknown_dist} and the case of the rectangles we will see subsequently, our analysis would need to not rely on the accuracy of the estimates but rather use these estimates to maintain progress or construct other versions of estimators that are unaffected by the adversarial injections.







\subsection{Generalizing Structure-based Algorithm beyond VC Dimension 1 Classes}

In \cref{sec:unknown_dist} we saw an algorithm that for any class $\mathcal{F}$ with VC dimension 1, achieves abstention and misclassification error bounded by $O(\sqrt{T})$ without access to the underlying distribution. An interesting open question is to extend structure-based algorithms beyond the VC 1 classes. Here we will show that for the class of axis-aligned rectangles in dimension $p$ (VC dimesnion is $2p$), we can indeed design an algorithm that achieves abstention and misclassification error bounded by $O(p\sqrt{T \log T})$. This exhibits a class of VC dimension $> 1$ for which we can attain the desired guarantees without access to the distribution.

Both our algorithms heavily utilize the structure of the underlying function class and analyze based on the notion of attackability. It would be interesting to characterize other structural hypothesis classes that enjoy similar guarantees. A natural extention to the axis-aligned rectangles would be any intersection closed hypothesis class.

\subsubsection{Structure-based Algorithm for Axis-aligned rectangles}
Recall that the class of axis-aligned rectangles consists of functions $f$ parameterized by $(a_1, b_1, \ldots,a_p, b_p)$ such that
\[
f_{(a_1, b_1, \ldots,a_p, b_p)}(x) = \begin{cases}
    1 & \text{ if } \forall i \in [p], a_i \le x_i \le b_i\\
    0 & \text{ otherwise.}
\end{cases}
\]

Now consider the following algorithm:

\begin{algorithm}[H] \label{alg:rectangles}
    \DontPrintSemicolon
    Set $a_1, \ldots, a_p = -\infty$ and $b_1, \ldots, b_p = \infty$ \\ 
    \For{$t=1,\ldots, T $  }{
        Receive $\postcorsamp{}$ \\ 
        \lIf{$\forall \tau <t, y_{\tau} = 0$}{
        $\hat{y}_t = 0$
        }
        \lElseIf{$\postcorsamp{} \notin \dis[1]( \cls_{t-1})$}{ $\hat{y_t} = f(\postcorsamp{})$ for any $f \in \cls_{t-1}$}
        \lElseIf{$\exists s_1 , \dots , s_{\alpha}  < t $ and $\exists i_1 , \dots , i_{\alpha} \in [p]$  such that $\hat{x}_{s_j,i_j}  \in [ \hat{x}_{t,i_j} , a_{i_j} ) \cup ( b_{i_j} , \hat{x}_{t,i_j} ]  $   }{$\pred = 0$}
        \lElse{$\pred = \bot$}
         Receiving label $y_t$\\
         Update $ \data \gets \data[t-1] \cup \left\{ ( \postcorsamp , y_t   )   \right\}   $ and $ \clst[t] \leftarrow \clstwpointo[t-1][\postcorsamp{}][y_t] $ \\
         Update $a_1, \ldots, a_p$ and $b_1, \ldots, b_p$ such that $ [a_1,b_1] \times \dots [a_p,b_p] $ is the smallest rectangle containing the points labelled positive so far. i.e. $a_i = \min \{ x_i : (x,1) \in S    \}    $
    }
    \caption{Structure-based learning for Axis-aligned Rectangles}
    \end{algorithm}
If we have only seen $0$ labels so far, the algorithm predicts $0$. Otherwise, let $[a_1,b_1] \times [a_2,b_2] \times \ldots \times [a_p,b_p]$ be the minimal rectangle enclosing the positive examples so far (i.e., the Closure hypothesis). For the next point $\postcorsamp{}$, if it isn't in the region of disagreement, we predict the agreed-upon label. Otherwise, we check whether there exist at least $\alpha$ examples $\hat{x}_s$, $s < t$, for each of which there exists a coordinate $i$ with $x_{si} \in [x_{ti},a_i) \cup (b_i,x_{ti}]$ (at most one of these sides is non-empty -- or sometimes both sides will be empty for some coordinates $i$). If so, we predict $0$. Otherwise, we abstain. (The algorithm never predicts 1 in the region of disagreement, similar to the Closure algorithm).
We formally capture the guarantees of the algorithm below:

\begin{theorem}
    Let $\cls$ be the class of axis aligned rectangles in $\mathbb{R}^p$. 
    Then, Algorithm~\ref{alg:rectangles} with $\alpha = \sqrt{T / \log T}  $ satisfies 
    \begin{align}
        \mathsf{Misclassification Error} &\le p \sqrt{T \log T}, \\ 
        \mathsf{AbstentionError} &\le  2p\sqrt{T\log T}  + 2p \log T.
    \end{align}
    




\end{theorem}


\begin{proof}
    For any example with target label 1, if the algorithm predicts $0$, there are at least $\alpha$ examples $\hat{x}_s$ which each have some coordinate $\hat{x}_{s,i}$ that was not in $[a_i,b_i]$ before the update, but which will have $\hat{x}_{s,i}$ in $[a_i,b_i]$ after the update. For each example $\hat{x}_s$, this can happen at most $p$ times (corresponding to each coordinate) before it will never again be included in a future set of $\alpha$ examples that convince us to predict $0$. So we make at most $pT/\alpha$ misclassifications on adversarially injected examples. Since the algorithm never predicts $1$ unless the true label is $1$, we never misclassify a negative example. So it remains only to bound the number of abstentions on the i.i.d. examples.

For any $n$, suppose $\hat{x}_t$ is the $n$-th i.i.d. example, and let $\tilde{x}_1,...,\tilde{x}_n$ be these $n$ i.i.d. examples (so $\tilde{x}_n = x_t$). If $x_t$ is "attackable" (same to \cref{def:atackable} meaning that there is some set of examples the adversary could add, knowing $\hat{x}_t$, to make us abstain) then it must be that either $\hat{x}_t$ is a positive example in the region of disagreement of the version space induced by the other $n-1$ points, or else $\hat{x}_t$ is a negative example such that there are $< \alpha$ points $\tilde{x}_{s}$, $s < n$, for which there exists $i$ with $\tilde{x}_{s,i} \in [x_{t,i},a_i) \cup (b_i,x_{t,i}]$. In particular, in the latter case, it must be that each coordinate $i$ has $< \alpha$ examples $\tilde{x}_{s}$ with $\tilde{x}_{s,i} \in [x_{t,i},a^*_i) \cup (b^*_i,x_{t,i}]$, where the target concept is $[a^*_1,b^*_1] \times \ldots \times [a^*_p,b^*_p]$. This is because the current estimated rectangle will be inside the true rectangle.

We will use exchangeability to bound the probability that $\tilde{x}_n$ is attackable by $\frac{1}{n}$ times the number of $\tilde{x}_s$, $s \leq n$, which would be attackable if they were swapped with $\tilde{x}_n$.  Among $\tilde{x}_1,\ldots,\tilde{x}_n$ there are at most $2p$ positive examples in the region of disagreement of the version space induced by the others (namely, the minimum spanning set of the positive examples). For each coordinate $i$, there are at most $2\alpha$ examples $\tilde{x}_s$, $s \leq n$, with $< \alpha$ other examples $\tilde{x}_{s',i}$ in $[\tilde{x}_{s,i},a^*_i) \cup (b^*_i,\tilde{x}_{s,i}]$ (namely, the $\leq \alpha$ examples with smallest $\tilde{x}_{s,i}$ such that $\tilde{x}_{s,i} > b^*_i$, and the $\leq \alpha$ examples with largest $\tilde{x}_{s,i}$ such that $\tilde{x}_{s,i} < a^*_i$). So there are at most $2\alpha p$ negative examples $\tilde{x}_{s}$ which would be attackable if they were swapped with $\tilde{x}_n$. 

Altogether there are at most $2p(\alpha+1)$ examples $\tilde{x}_{s}$ which would be attackable if they were swapped with $\tilde{x}_n$. Thus, the probability i.i.d. example $\hat{x}_t$ is attackable is at most $2p(\alpha+1)/n$ where $n$ is the number of i.i.d. points seen so far including $\hat{x}_t$. Summing, the expected number of abstentions on i.i.d. examples is at most $2p(\alpha+1)\log T$. Now setting $\alpha = \sqrt{T/\log T}$, gives us the desired result. 
\end{proof}
